From Discrete to Continuous Convolution Layers

A basic operation in Convolutional Neural Networks (CNNs) is spatial resizing of feature maps. This is done either by strided convolution (donwscaling) or transposed convolution (upscaling). Such operations are limited to a fixed filter moving at predetermined integer steps (strides). Spatial sizes of consecutive layers are related by integer scale factors, predetermined at architectural design, and remain fixed throughout training and inference time. We propose a generalization of the common Conv-layer, from a discrete layer to a Continuous Convolution (CC) Layer. CC Layers naturally extend Conv-layers by representing the filter as a learned continuous function over sub-pixel coordinates. This allows learnable and principled resizing of feature maps, to any size, dynamically and consistently across scales. Once trained, the CC layer can be used to output any scale/size chosen at inference time. The scale can be non-integer and differ between the axes. CC gives rise to new freedoms for architectural design, such as dynamic layer shapes at inference time, or gradual architectures where the size changes by a small factor at each layer. This gives rise to many desired CNN properties, new architectural design capabilities, and useful applications. We further show that current Conv-layers suffer from inherent misalignments, which are ameliorated by CC layers.

==> 07_broader_impact.tex <==
\section*{Broader Impact}
% This work does not present any foreseeable societal consequence.

% The dynamic features of the new CC-layer has the potential to replace multiple network (for example SR networks for different scales) with a single network, which may yield both better results and may save resources (especially electricity).

\textbf{\it Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
Authors should discuss both positive and negative outcomes, if any.} \\

\underline{\textbf{AUTHORS' ANSWER:}}

\textbf{a) Who may benefit from this research?}
Any ML or CV researcher, or code developer, who uses Deep Learning code and designs neural architectures.

\textbf{b) Who may be put at disadvantage from this research?}
No one, to our best knowledge.

\textbf{c) What are the consequences of failure of the system?}
Not applicable. This is not a system, but rather a new useful component in Deep Learning architectures.

\textbf{d) Whether the task/method leverages biases in the data?}
Not to our best knowledge.

